Interpolation-Aware Padding for 3D Sparse Convolutional Neural Networks

Sparse voxel-based 3D convolutional neural networks (CNNs) are widely used for various 3D vision tasks. Sparse voxel-based 3D CNNs create sparse non-empty voxels from the 3D input and perform 3D convolution operations on them only. We propose a simple yet effective padding scheme --- interpolation-aware padding to pad a few empty voxels adjacent to the non-empty voxels and involve them in the 3D CNN computation so that all neighboring voxels exist when computing point-wise features via the trilinear interpolation. For fine-grained 3D vision tasks where point-wise features are essential, like semantic segmentation and 3D detection, our network achieves higher prediction accuracy than the existing networks using the nearest neighbor interpolation or the normalized trilinear interpolation with the zero-padding or the octree-padding scheme. Through extensive comparisons on various 3D segmentation and detection tasks, we demonstrate the superiority of 3D sparse CNNs with our padding scheme in conjunction with feature interpolation.

==> src/tables/padding-numbers.tex <==
\begin{table}[h]
    \centering
    \scalebox{0.7}{
    \begin{tabular}{rrrrr}
        \toprule
                       & $s=1/10$ & $s=1/20\,$ & $s=1/40\;$ & $s=1/80\quad$ \\
        \midrule
        zero padding     & $1236|1325$        & $4274|\;\;5096$        & $9686|19085$       & $9952|\;\;62890$       \\
        1-ring padding & $3868|3943$        & $14908|15608$     & $56204|62387$      & $182397|240188$    \\
        octree padding & $2488|2600$        & $9488|10184$       & $34120|40656$      & $77448|152904$     \\
        fea. padding   & $2425|2501$        & $9579|10309$       & $34172|40680$      & $77321|152110$     \\
        \bottomrule
    \end{tabular}
    }
    \caption{The total voxel number under different padding strategies for the 3D point set sampled from a Bunny model. Number $A$ and $B$ with form ``$A|B$'' denote the voxel number under the setup of $10000$ input points and $100000$ input points, respectively.
    }
    \label{tab:voxelnumber}
\end{table}

==> src/tables/partnet-detail.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.8}{
        \begin{tabular}{c|rrrr}
            \toprule
            \thead{Item}      & \thead{Chair} & \thead{Lamp} & \thead{Stora} & \thead{Table} \\
            \midrule
            Train Data      &  4489  & 1554 & 1588 & 5707  \\
            Val Data        &   617  & 234  &  230 &  843  \\
            Test Data       &  1217  & 419  &  451 & 1668  \\
            Epochs          &   140  & 200  &  200 &  110  \\
            \bottomrule
        \end{tabular}
    }
    \caption{Details of the PartNet Segmentation Task.}  \label{tab:partnet_details}
\end{table}


==> src/tables/partnet-seg.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.8}{
        \begin{tabular}{cccccrr}
            \toprule
            \thead{Group}        & \thead{Network} & \thead{Conv} & \thead{Int} & \thead{mIOU}  & \thead{Time}  & \thead{Mem}   \\
            \midrule
            \multirow{4}{*}{(1)} & ZP-UNet         & I            & Near.       & $40.5\pm0.2$  & 71            & 424           \\
                                 & NP-UNet         & I            & Near.       & $40.9\pm0.0$  & 95            & 1313          \\
                                 & OP-UNet         & I            & Near.       & $40.0\pm0.0$  & 81            & 879           \\
                                 & IP-UNet         & I            & Near.       & $40.6\pm0.1$  & 88            & 903           \\
            \midrule
            \multirow{4}{*}{(2)} & ZP-UNet         & I            & Norm.       & $41.5\pm0.0$  & 131           & 446           \\
                                 & NP-UNet         & I            & Norm.       & $42.7\pm0.3$  & 298           & 1327          \\
                                 & OP-UNet         & I            & Norm.       & $41.4\pm0.0$  & 195           & 881           \\
                                 & IP-UNet         & I            & Norm.       & $42.3\pm0.3$  & 205           & 906           \\
            \midrule
            \multirow{2}{*}{(3)} & ZP-UNet         & I            & UNorm.      & $39.3\pm0.1$  & 123           & 446           \\
                                 & OP-UNet         & I            & UNorm.      & $40.6\pm0.0$  & 193           & 881           \\
            \midrule
            \multirow{4}{*}{(4)} & ZP-UNet         & II           & Near.       & $39.6\pm0.0$  & 189           & 423           \\
                                 & NP-UNet         & II           & Near.       & $40.8\pm0.0$  & 378           & 1310          \\
                                 & OP-UNet         & II           & Near.       & $39.3\pm0.0$  & 271           & 879           \\
                                 & IP-UNet         & II           & Near.       & $39.9\pm0.0$  & 282           & 903           \\
            \midrule
            \multirow{4}{*}{(5)} & ZP-UNet         & II           & Norm.       & $41.1\pm0.0$  & 198           & 446           \\
                                 & NP-UNet         & II           & Norm.       & $41.7\pm0.0$  & 391           & 1328          \\
                                 & OP-UNet         & II           & Norm.       & $41.0\pm0.0$  & 274           & 882           \\
                                 & IP-UNet         & II           & Norm.       & $41.3\pm0.0$  & 289           & 906           \\
            \midrule
            \multirow{2}{*}{(6)} & OP-UNet\textsuperscript{+}         & I           & Norm.       & \textred{???} & 216 & 1110 \\
                                 & IP-UNet\textsuperscript{+}         & I           & Norm.       & \textred{???} & 211 & 975  \\
            \bottomrule
        \end{tabular}
    }
    \caption{ Quality statistics of fine-grained segmentation on four PartNet categories under different settings. \emph{Conv} is the sparse convolution type, \emph{Int} is the sparse interpolation type, \emph{mIOU} is the average part IOU, \emph{Time} is the average time in milliseconds of a single forward and backward propagation on a batch  (16 objects), and \emph{Mem} is the average GPU memory (in Megabyte) occupied by a batch. The experiments are grouped for analysis. \todo{update number, hightlight the best number in each group}}  \label{tab:partnetseg} %\vspace{-4mm}
\end{table}

